Robots That Ask For Help: Uncertainty Alignment for Large Language Model Planners

Large language models (LLMs) exhibit a wide range of promising capabilities -- from step-by-step planning to commonsense reasoning -- that may provide utility for robots, but remain prone to confidently hallucinated predictions. In this work, we present KnowNo, which is a framework for measuring and aligning the uncertainty of LLM-based planners such that they know when they don't know and ask for help when needed. KnowNo builds on the theory of conformal prediction to provide statistical guarantees on task completion while minimizing human help in complex multi-step planning settings. Experiments across a variety of simulated and real robot setups that involve tasks with different modes of ambiguity (e.g., from spatial to numeric uncertainties, from human preferences to Winograd schemas) show that KnowNo performs favorably over modern baselines (which may involve ensembles or extensive prompt tuning) in terms of improving efficiency and autonomy, while providing formal assurances. KnowNo can be used with LLMs out of the box without model-finetuning, and suggests a promising lightweight approach to modeling uncertainty that can complement and scale with the growing capabilities of foundation models. Website: https://robot-help.github.io

==> old/sections/experiments.tex <==
\section{Experiments}
% We hope to address the following questions through extensive experiments of different robotic tasks:
% \begin{enumerate}
%     \item 
% \end{enumerate}

% \textbf{Questions:}
% \begin{enumerate}
%     \item Can our method improve performance compared to Sys-ID approaches when the target is out of domain in simulation and in real? Different amount of real data
%     \item Can our method be more efficient (requiring fewer trials) when adapting to target either within or out of domain?
%     \item Can our method at least match the performance of Sys-ID approaches when the target is within domain in simulation?
% \end{enumerate}

\paragraph{Baselines:} (1) Naive; (2) Conformal Top-k; (3) LLM directly outputting prediction set; (4) Ensemble...


==> old/sections/formulation.tex <==
\section{Problem formulation}

\paragraph{Environment.} Each environment, denoted $E$, is sampled from some distribution $\mathcal{D}_{E}$. The environment can be a table-top setup with multiple objects and a robotic arm. The environment distribution can then represent the distribution of the initial poses of the objects.

\paragraph{Time step.} There are two types of ``steps'' in play: both cases involve the robot doing some prediction, but in one case the robot predicts so that it can take an action, and in other case the robot predicts to determine if it is uncertain about the action and asks a clarification question to human.
% the step of the robot taking an action (\eg move a block and place it somewhere), and the step of the robot predicting the correct action to take and possibly asking the question to human if its prediction is uncertain. 
The robot may interact with human multiple times to fully understand the human intention before taking an action.
% and thus there are more steps of predictions than actions.
For now we do not differentiate these two different types of steps and denote the time step $t$. We may drop the superscript $t$ in the single-step setting.

\paragraph{State.} We denote the state at step $t$ as $s^t$; in the table-top manipulation setting, it includes the poses of the objects on the table.

\paragraph{Context.} The robot needs information of the current state and the task in the text format, which is fed into the LLM for action planning at each step. We call such text descriptions context, denoted $x^t$. The context can potentially summarize the current state, \eg ``there are a blue bowl and yellow block on the table'', the previous actions taken by the robot, \eg ``in the last step, you put the green block to the left of the yellow bowl,'' the task, \eg ``put a yellow bowl next to the blue block, '' and some additional information such as an example, \eg ``to put ... at ..., you would first ..., then ...'' For now, we assume the state is fully grounded; either the visual scene is fully described in the context (using a visual-language model such as ViLD), or the robot can have access to the true locations of the objects when executing the action (\eg through API functions such as \verb|get_obs_pos(obj_name)|).

\paragraph{LLM planner and action.} We assume there is a LLM-based planner that maps the context to the robot action $a^t$ (\eg pick-and-place an object) at a step, denoted $\pi: x^t \mapsto a^t$. Note the robot may not take an action at a certain step since it could only interact with humans for clarification. For now, we assume the action is always executed successfully (\ie the object is moved to the desired location specified by the planner output without moving the other objects).

\paragraph{Task.} The task is defined with a reward function $R$, \eg 1 if all objects specified in the request are moved to the correct locations, and 0 otherwise. The task is conveyed to the robot in the format of text request, \eg ``put three blocks next to the yellow bowl.''

\TODO{have a dedicated paragraph here on the different data distributions.}


==> old/sections/introduction.tex <==
\section{Introduction}

LLM planners have shown success in planning long-horizon action sequences of the robot. However, when the task is ambiguous (\eg ``fetch me a beverage from the fridge'', but what kind of beverage?) or the task is difficult, the LLM planner can be uncertain about the plan. It is important to model the uncertainty of the LLM planner in these cases, such that humans can offer help if needed by providing clarifications or directly providing the correct actions. As such, we want to improve the success rate of the robot completing the tasks.

This is also related to the value alignment problem: we want the LLM to learn to align with the human intention --- clarifying the ambiguities in the task request, but do not ``overthink'' by considering potential ambiguities that humans are not concerned with (\eg the orientation of the block/bowl).

Conformal prediction is a classic method that allows us to formally model the uncertainty of the LLM planner by generating prediction sets. The benefit of using conformal prediction is twofold: (1) the prediction results are calibrated (\ie representing the true probability of each option), and (2) it provides guarantees for test samples from the same distribution of the training ones. We can trigger robot asking for help when, \eg the prediction set is not a singleton.

Contributions:
\begin{itemize}
    \item Curate a dataset of ambiguous requests, multiple choices, and the ground-truth answer
    \item Propose using conformal prediction... improve empirical coverage... in ambiguous settings
    \item Provide end-to-end guarantee for the whole sequence in multi-step setting
    \item Provides (conditional) coverage guarantee...
\end{itemize}


==> old/sections/preliminaries.tex <==
\section{Preliminaries}

\subsection{LLM Planning as Multiple Choice (Generation and) Answering.}

Conformal prediction assumes that the LLM planner returns meaningful uncalibrated scores for each step of the plan.
For image classification, this is as simple as the class category softmax scores, but for LLMs this is a bit more tricky. LLM planners are usually autoregressive models, which means they predict each step token by token. We can get softmax scores for each token. But to get a single score for a sequence of tokens, we need perplexity. However, perplexity is a poor scoring function because it biases against longer steps with lower values.

One simple workaround for this involves some creative prompting: formulate step selection as a multiple choice Q\&A problem. We can first use a standard LLM-based planner + beam search to generate multiple candidate next steps in a plan. Then, we ask the same LLM to choose among the candidates with multiple choices. This reduces step selection as a single-token prediction problem.

The multiple choices at each step can be generated either with templates or by prompting the LLM.

\paragraph{Label.} For each step, there is at least one true action. To always cover the true action with the multiple choices at each step, we will consider four options generated with the template or by prompting, plus a fifth option ``none of the other options''. By assigning higher biases to tokens of $[a, b, c, d ,e]$ (with \verb|logit_bias| argument in \verb|openai.Completion.create()| function for GPT-3) and setting the maximum length to be 1, we can constrain the LLM to always output one of the five letters. We define the label of each prediction as the true option among the five, denoted $y$. We will extend to multi-label setting later.

% (\eg the task is to ``put two blocks to the left of the yellow bowl'' and we consider the true action in the first step is to ``put the blue block ...'' this is an interesting case, since ideally ``put the yellow block ...'' is also correct, and we should not consider this ambiguous)

\subsection{Single-Step Conformal Prediction.}

For the single-step case, we follow the typical conformal prediction procedure. We collect a dataset $S = \{(x_i, y_i) \}_{i=1}^N$ containing inputs and their correct labels. Each sample in $S$ is a trial of request/context and the true answer. These examples are drawn from a distribution $\mathcal{D}$ where the environment is randomly initialized, and an instruction for a task is randomly provided. For context $x$, we have some heuristic notion of confidence over labels (\eg softmax values of token predictions of the LLM):
\begin{equation}
    \hat{f}(x) \in [0,1]^{\RR_K},
\end{equation}
where $K=5$ in the current setup. We denote the confidence for a particular label $y$ as $\hat{f}(x)_{y}$. With this, we can proceed with the usual conformalization procedure. Define the calibration scores:
\begin{equation}
    s_i := 1-\hat{f}(x_i)_{y_i}, i=1,...,N.
\end{equation}

Define $\hat{q}$ to be the $\frac{\lceil (n+1)(1-\alpha) \rceil}{n}$ empirical quantile of $s_1, ..., s_n$. For a new test sample $x_\text{test}$ drawn from the same distribution as samples in $S$, define the prediction set:
\begin{equation}
    C(x_\text{test}) := \{y \ | \ \hat{f}(x_\text{test})_{y} \geq 1-\hat{q} \}.
\end{equation}

Conformal prediction then provides the bound that $\PP(y_\text{test} \notin C(x_\text{test})) \leq \alpha$.

\subsection{Multi-Step Conformal Prediction by Lifting to Sequences.}

Often the setting we consider involves multiple robot actions in sequence (\eg asking a mobile robot to fetch a coke from the refrigerator in the kitchen involves drive to the kitchen, find the fridge, open the door, ...). In addition, with human providing clarifications after the robot asks questions, the robot would make multiple rounds of action prediction. Such multi-step scenarios involve prediction over steps in a trial that are correlated, breaking the i,i,d. requirement of the usual conformal prediction.

One way to address the issue is to lifting the problem to sequences: we provide end-to-end conformal prediction guarantee for the whole sequence instead of for individual steps. Our approach has three steps: (i) \emph{lifting} the problem to sequences, (ii) performing \emph{conformal prediction} in the space of sequences, and (iii) \emph{causal reconstruction} of the sequence-based prediction sets during test time. 

\paragraph{Part 1: Lifting to sequences.}

Each trial involves a sequences of contexts:
\begin{equation}
    \olsi{x} = (x^0, x^1, ..., x^{T-1})
\end{equation}
and labels:
\begin{equation}
    \olsi{y} = (y^0, y^1, ..., y^{T-1})
\end{equation}

We collect a dataset $\olsi{S} = \{ (\olsi{x}_i, \olsi{y}_i) \}_{i=1}^N$. Each sample in $S$ is the requests/contexts and the true answers over multiple steps in one trial. These examples are drawn from a distribution $\olsi{\mathcal{D}}$ where the environment is randomly initialized, an instruction for a task is randomly provided, and context $x^t$ arise from having done the \textbf{correct} actions in previous steps.

At test time, we follow the following process:
\begin{algorithm}[H]
\caption{Multi-step LLM planning with human help.}
\small
\begin{algorithmic}[1]
    % \Require $E^r$, real environment
    \vspace{1mm}
    %
    \For{time $t \leftarrow 0$ to $T-1$}
    \State Observe input $x_\text{test}^t$
    \State Predict a set $C(x_\text{test}^t)$
    \If{$C(x_\text{test}^t)$ is a singleton}
        \State execute corresponding action
    \Else
        \State ask for help, which is always assumed to provide the correct label, or the human provide clarification only
    \EndIf
\EndFor
% \Return $\pi^*_{\mathcal{E}_i}$ with the highest $R(\cdot; E^r)$
\end{algorithmic}
\normalsize
\label{algo:adaptation}
\end{algorithm}

Define $C(\olsi{x}_\text{test}) := C^0(x_\text{test}^0) \times C^1(x_\text{test}^1) \times ... \times C^{T-1}(x_\text{test}^{T-1})$. Let $\olsi{y}_\text{test}$ be the sequence of true labels for $\olsi{x}_\text{test}$. Our goal is to provide a bound:
\begin{equation}
    \PP(\olsi{y}_\text{test} \notin C(\olsi{x}_\text{test})) \leq \alpha.
\end{equation}

This is a lower bound $(1-\alpha)$ on the end-to-end success rate (since a failure only happens when the prediction set is singleton containing the wrong label; this probability is $\leq \alpha$).

\paragraph{Part 2: Conformal prediction.}

For context $x^t$ at each step, we apply the same heuristic notion of confidence over labels, $\hat{f}(x^t) \in [0,1]$. We denote the confidence for a particular label $y^t$ as $\hat{f}(x^t)_{y^t}$. Using this, we will define a heuristic notion of confidence for an entire sequence:
\begin{equation}
    \hat{f}(\olsi{x})_{\olsi{y}} := \min_t \ \hat{f}(x^t)_{y^t}.
\end{equation}

With this, we can proceed with the usual conformalization procedure. Define the calibration data sequences:
\begin{equation}
    s_i := 1-\hat{f}(\olsi{x}_i)_{\olsi{y}_i}, i=1,...,N.
\end{equation}

Define $\hat{q}$ to be the $\frac{\lceil (n+1)(1-\alpha) \rceil}{n}$ empirical quantile of $s_1, ..., s_n$. For a new test sequence $\olsi{x}_\text{test}$ drawn from the same distribution as the sequences in $S$, define:
\begin{equation}
    \olsi{C}(\olsi{x}_\text{test}) := \{ \olsi{y} \ | \ \hat{f}(\olsi{x}_\text{test})_{\olsi{y}} \geq 1-\hat{q} \}.
\end{equation}

In words, $\olsi{C}(\olsi{x}_\text{test})$ is a set of prediction sequences (\eg \{(a,b,c), (b,c,c), ...\} with $T=3$). Conformal prediction then provides the bound that $\PP(\olsi{y} \notin \olsi{C}(\olsi{x}_\text{test})) \leq 1-\alpha$.

\paragraph{Part 3: Causal construction.}
% , and thus we cannot obtain the score function of the sequence $\hat{f}(\olsi{x})_{\olsi{y}}$
The main challenge now is that at test time, we do not see the entire sequence $\olsi{x}_\text{test}$ all at once. Rather, we see context $x_\text{test}^t$ one at a time. We thus need to be able to construct (or over-approximate) $\olsi{C}(\olsi{x}_\text{test})$ in a \underline{causal} manner (\ie always replying only on current/past information).

Let's call $C(\olsi{x}_\text{test})$ the causally reconstructed prediction set at time $t$, which we define as:
\begin{equation}
    C^t(x_\text{test}^t) := \{ y^t \ | \ \hat{f}(x_\text{test}^t)_{y^t} \geq 1-\hat{q} \}.
\end{equation}

\noindent \textbf{Claim:} suppose that for a test sequence $\olsi{x}_\text{test}$, the true label $\olsi{y}_\text{test}$ belongs to $\olsi{C}(\olsi{x}_\text{test})$. Then, $\olsi{y}_\text{test}$ also belongs to $C(\olsi{x}_\text{test})$. Thus, since we can bound the probability that $\olsi{y}_\text{test} \notin \olsi{C}(\olsi{x}_\text{test})$, we can also bound the probability that $\olsi{y}_\text{test} \notin C(\olsi{x}_\text{test})$, which in turn provides a guarantee on the end-to-end performance (by the argument provided at the end of Part 1 earlier).

\noindent \textbf{Proof:} suppose $\olsi{y}_\text{test} \in \olsi{C}(\olsi{x}_\text{test})$. Then, by definition of $\olsi{C}(\olsi{x}_\text{test})$, we have:
\begin{equation}
    \min_t \ \hat{f}(x_\text{test}^t)_{y_\text{test}^t} \geq 1-\hat{q}.
\end{equation}
Thus, for all $t$:
\begin{equation}
    \hat{f}(x_\text{test}^t)_{y_\text{test}^t} \geq 1-\hat{q}.
\end{equation}
Hence, for all $t$:
\begin{equation}
    y_\text{test}^t \in C^t(x_\text{test}^t).
\end{equation}
Finally, $\olsi{y}_\text{test} \in C(\olsi{x}_\text{test})$.

\paragraph{Overall procedures:}
\begin{itemize}
    \item Run conformal prediction with $S$ and the score function $\hat{f}(\olsi{x})_\olsi{y}$. Obtain the guarantee $\PP(\olsi{y} \in \olsi{C}(\olsi{x}_\text{test})) \geq 1-\alpha$ with quantile $\hat{q}$.
    \item At test time, construct the prediction set $C(\olsi{x}_\text{test})$ incrementally at each step with $C^t(x_\text{test}^t)$. Since we prove that if $\olsi{y}_\text{test} \in \olsi{C}(\olsi{x}_\text{test})$ then $\olsi{y}_\text{test} \in C(\olsi{x}_\text{test})$, then we have the guarantee $\PP(\olsi{y} \in C(\olsi{x}_\text{test})) \geq 1-\alpha$.
\end{itemize}

Thus, we obtain guarantee for $C(\olsi{x}_\text{test})$ without running calibration using per-step data, which would have required $x^t$ being i,i,d.

\paragraph{Underlying data distribution:}
Let's be clear about the underlying distribution of the context and label sequence. Notice that the context and label at each step can depend on those from previous steps (\eg the order of moving the objects matters). Thus we can consider a distribution of the initial context and label $\mathcal{D}^0$. If we sample an initial pair $(x^0, y^0) \sim \mathcal{D}^0$, then $(x^t, y^t) = q(x^{t-1}, y^{t-1})$, where $q$ is some function capturing the LLM and human-LLM interaction, and does not depend on other calibration data sequences (no need to include steps earlier than $t-1$ since $x^{t-1}$ already summarizes all previous steps). Thus we can reduce sampling i,i,d. from $\mathcal{D}$ to sampling i,i,d. from $\mathcal{D}^0$ instead. $q$ can also be stochastic as both LLM and human can be non-deterministic, then it is reduced to sampling i,i,d. from $\mathcal{D}^0$ and from the conditional distribution at each step. The probability of the sequence can be expressed as:
\begin{equation}
    f_{(\olsi{X}, \olsi{Y})}(\olsi{x}, \olsi{y}) = p((x^0, y^0))\prod_{t=1}^{T-1} p((x^t, y^t) | (x^{t-1}, y^{t-1}))
\end{equation}

\subsection{Extending to multi-label setting}
\label{subsec:single-step-multi-label}

Often we encounter scenarios where there can be multiple true labels in one time step: for example, the task is to ``put three blocks in the yellow bowl'', and for the first step, moving any of the blue/yellow/green block should be treated as correct. We would like to have an end-to-end guarantee that states, for example, with 95\% probability over test sequences, for each step of a test sequence, there is at least one true label included in the prediction set. 

Let's first consider the single-step setting. We have a dataset of $S = \{(x_i, Y_i),...\}_{i=1}^N$ sampled i,i,d. from a data distribution $\mathcal{D}$ for calibration (we use the same notation $\mathcal{D}$ as in the single-label setting here), where $Y_i := \{y_{i,j}\}_{j=1}^{J_i}$ is the set of true labels for a single trial. For each label, we use the same heuristic notion of confidence, $\hat{f}(x)_y \in [0,1]$.

Next, we define an operator $\beta: \mathcal{X} \times \mathcal{Y}^K \rightarrow \mathcal{Y}$ where $\mathcal{X}$ is the space of context and $\mathcal{Y}$ is the space of labels:
\begin{equation}
    \beta(x, Y) := \arg \max_{y \in Y} \hat{f}(x)_y,
\end{equation} 
which takes the true label with the highest confidence value from the true label set.

If we consider applying $\beta$ to every point in the support of $\mathcal{D}$, a new distribution $\mathcal{D}'$ is induced. We also consider $S' = \{ (x_i, y^{\max}_i) \}_{i=1}^N$, where $ y^{\max}_i := \beta(x_i, Y_i)$. Then we can perform the usual conformalization and obtain the guarantee that with
\begin{equation}
    C(x_\text{test}) := \{y | \hat{f}(x_\text{test})_y \geq 1-\hat{q}\},
\end{equation}
then:
\begin{align}
    \PP(y^{\max}_\text{test} \notin C(x_\text{test})) &\leq \alpha, \\
    \PP(\arg \max_{y \in Y_\text{test}} \hat{f}(x_\text{test})_y \notin C(x_\text{test})) &\leq \alpha, \\
    \PP(\beta(x_\text{test}, Y_\text{test}) \notin C(x_\text{test})) &\leq \alpha,
\end{align}
which is the desired guarantee. At test time, we sample $(x_\text{test}, Y_\text{test})$ from $\mathcal{D}$ that is i,i,d. with samples in $S$ ---  for the guarantee to hold for $\beta(x_\text{test}, Y_\text{test})$, we need to show $\beta(x_\text{test}, Y_\text{test})$ is a sample from $\mathcal{D}'$ that is i,i,d. with samples in $S'$. This is true since functions of independent random variables are independent, and functions of identically distributed random variables are identically distributed if the functions are measurable.

\begin{remark}There is the subtlety that data distribution $\mathcal{D}'$ depends on the heuristic $\hat{f}(x)_y$, but the proof of conformal prediction guarantee does not assume independence between the data distribution and the heuristic (score function).\end{remark}

\subsection{Multi-label multi-step setting}

For the multi-step setting, each trial now involves a sequence of contexts $\olsi{x}$ and a set of sequences of true labels:
% a sequence of sets of true labels
% \begin{equation}
%     \olsi{Y} = (Y^0, Y^1, ..., Y^{T-1}).
% \end{equation}
\begin{equation}
    \olsi{Y} = \{ \olsi{y}_1, \olsi{y}_2, ..., \olsi{y}_{M} \},
\end{equation}
where $\olsi{y}_m := (y^1_m, y^2_m, ..., y^{T-1}_m)$. For example, $\olsi{Y}$ can contain the sequence of ``blue block, yellow block, green block'', ``green block, blue block, yellow block'', ..., for the task of picking up three blocks. We collect a dataset of $\olsi{S} = \{(\olsi{x}_i, \olsi{Y}_i)\}$ of i,i,d. samples from the data distribution $\olsi{\mathcal{D}}$.

Unlike the single-step setting in Sec.~\ref{subsec:single-step-multi-label}, here we cannot apply $\beta$ to the set of true labels in each step, since we are considering a set of sequences of true labels, instead of a sequence of sets of true labels, because the true label set at time step $t$ depends on the set at the previous step $t-1$.

Instead, we introduce a slightly different (autoregressive) operator $\olsi{\beta}_t: \mathcal{X} \times \olsi{\mathcal{Y}^K} \rightarrow \olsi{\mathcal{Y}}$ where $\olsi{\mathcal{Y}}$ is the space of sequence of labels \allen{the notations here can be improved}:
\begin{align}
    \olsi{\beta}_t(\olsi{x}, \olsi{Y}) := \{ \arg \max_{y \in Y^\tau} \hat{f}(x)_y \}, & \ \tau=1,...,t-1, \\
    & \text{where} \ Y^\tau := \{ y^t_m \} \ \text{if} \ \olsi{\beta}_{\tau-1}(\olsi{x}, \olsi{Y}) = \{ \olsi{y}^t_m \}_{t=1}^{\tau-1}.
\end{align}

For convenience, we denote $\olsi{\beta}_t(\olsi{x}, \olsi{Y})[\tau]$ the $\tau$ element in $\olsi{\beta}_t(\olsi{x}, \olsi{Y}), \tau \leq t$. An intuitive interpretation is that, we can consider $\olsi{Y}$ forming a tree of valid executions:

\begin{figure}[H]
\centering
\includegraphics[width=0.50\textwidth]{sections/label-tree.png}
% \vspace{-5mm}
% \caption{Overview.}
% \label{fig:diagram}
\end{figure}

And $\olsi{\beta}_T(\olsi{x}, \olsi{Y})$ prunes the tree to a single branch by taking the true label with the highest heuristic value $\hat{f}(x^t)$ at each step:

\begin{figure}[H]
\centering
\includegraphics[width=0.15\textwidth]{sections/tree-pruning.png}
% \vspace{-5mm}
% \caption{Overview.}
% \label{fig:diagram}
\end{figure}

 % Consider $C(\olsi{x}_\text{test}) := C^0(x_\text{test}^0) \times C^1(x_\text{test}^1) \times ... \times C^{T-1}(x_\text{test}^{T-1})$ causally constructed, where $C^t(x^t_\text{test}) &= \{ y^t | \hat{f}(x^t_\text{test})_{y^t} \geq 1-\hat{q} \}$.

Now we can again apply $\olsi{\beta}_T$ to every point in the support of $\olsi{\mathcal{D}}$, a new distribution $\olsi{\mathcal{D}}'$ is induced. We consider $\olsi{S}' = \{(\olsi{x}_i, \olsi{y}^{\max}_i)\}$, where $ \olsi{y}^{\max}_i := \olsi{\beta}_T(\olsi{x}_i, \olsi{Y}_i)$. Let $\olsi{Y}_\text{test}$ be the set of sequences of true labels for $\olsi{x}_\text{test}$. Suppose we get the bound with $\olsi{\beta}_T$ as the labels:
\begin{equation}
    \PP(\olsi{\beta}_T(\olsi{x}_\text{test}, \olsi{Y}_\text{test}) \notin C(\olsi{x}_\text{test})) \leq \alpha,
\label{eq:bound-multi-label-multi-step}
\end{equation}
which states that at test time, given a context sequence $\olsi{x}_\text{test}$, we produce a prediction set sequence; if we consider a sequence consisting of the true label with the highest score at each step, the probability of this sequence covered by $C(\olsi{x}_\text{test})$ is lower bounded by $1-\alpha$. However, we need to be careful of following $\olsi{\beta}_t$ at each step at test time. Conside the three cases:
\begin{itemize}
    \item (1) At a given time-step, the prediction set $C^t(x^t_\text{test})$ does not contain the true label, $\olsi{\beta}_t(\olsi{x}, \olsi{Y})[t]$
    \item (2a) The prediction set is a singleton and does contain the true label
    \item (2b) The prediction set is not a singleton (but does contain the correct label)
\end{itemize}

We already bound the probability of (1) happening with the bound; (2a) is fine since the LLM will take the correct action; (2b) is tricky --- in this case the robot asks the human for help, and we need to make sure the human ``follows'' the true label, by choosing the true label in the prediction set with the highest confidence by $\hat{f}$.

% Then we can perform the usual conformalization and obtain the guarantee that with
% \begin{equation}
%     C(\olsi{x}_\text{test}) := \{y | \hat{f}(x_\text{test})_y \geq 1-\hat{q}\},
% \end{equation}

% We further extend $\beta$ to multi-step setting by defining:
% \begin{equation}
%     \olsi{\beta}(\olsi{x}, \olsi{Y}) := \{\arg \max_{y \in Y^t} \hat{f}(x^t)_y\}, t=1,...,T-1.
% \end{equation}


Now let's derive the bound in Eq.~\eqref{eq:bound-multi-label-multi-step}. Again we need to deal with the causal reconstruction issue. 
% During calibration, we consider the new distribution $\olsi{\mathcal{D}}'$ by applying $\olsi{\beta}$ to every support of $\olsi{\mathcal{D}}$, and the new dataset $\olsi{S}' = \{(\olsi{x}_i, \olsi{y}^{\max}_i\}_{i=1}^N$, where $\olsi{y}^{\max}_i := \olsi{\beta}(\olsi{x}_i, \olsi{Y}_i)$. 
We construct the prediction set $\olsi{C}(\olsi{x}_\text{test})$ non-causally using the score function $s_i = 1-\hat{f}(\olsi{x}_i)_{\olsi{y}^{\max}_i}$ (taking minimum over steps). For a test sequence $\olsi{x}_\text{test}$, we apply $\olsi{\beta}_T$ to the true label set sequence $\olsi{Y}_\text{test}$ to get $ \olsi{y}^\text{max}_\text{test} = \olsi{\beta}_T(\olsi{x}_\text{test}, \olsi{Y}_\text{test})$. Now suppose $\olsi{y}^\text{max}_\text{test} \in \olsi{C}(\olsi{x}_\text{test})$, then we can show $\olsi{y}^\text{max}_\text{test} \in C(\olsi{x}_\text{test})$ with the same proof as the single-label setting, which gives us the bound.

Lastly we need to show the sampled test sequence from $\olsi{D}$ leads to a sample from $\olsi{\mathcal{D}}'$ i,i,d. with $\olsi{S}'$. This is true with the same argument that functions of independent random variables are independent.

% To do so, we can consider the initial pair $(x^1_\text{test}, Y^1_\text{test})$ an i,i,d. sample from $\mathcal{D}^1$. Then the corresponding $\beta(x^1_\text{test}, Y^1_\text{test})$ is also an i,i,d. sample from $\mathcal{D}'^1$ as demonstrated earlier. The whole sequence $(\olsi{x}_\text{test}, \olsi{Y}_\text{test})$ can be considered as a function of $(x^1_\text{test}, Y^1_\text{test})$, and since functions of independent random variables are independent, 

% Then we modify the heuristic notion of confidence for the trial:
% \begin{equation}
    % \tilde{f}(x)_{\tilde{y}} := \max_j \hat{f}(x)_{y_j}.
% \end{equation}

% To provide such guarantee, first we denote the set of all true labels at a time step as $\tilde{y}^t := \{y^t_j\}_{j=1}^{J}$. The sequence of the set of true labels over steps is $\tilde{y} = (\tilde{y}^0, \tilde{y}^1, ..., \tilde{y}^{T-1})$. We then define the all sequences of individual true label as the Cartesian product of $\tilde{y}^t$: $S_{\tilde{y}} := \tilde{y}^0 \times \tilde{y}^1 \times ... \times \tilde{y}^{T-1}$. 

% \allen{seemingly $S_{\tilde{y}}$ is not the true set of sequences of true labels: $\tilde{y}^t$ can depend on $\tilde{y}^{t-1}$, \eg moving the blue block for the first step means in the second step, it is no longer a true option. However, we assume that true labels are defined in a time-dependent way already. We can think of that the true labels at each time step are incrementally determined as the sequence proceeds.}

% % Then we modify the heuristic notion of confidence over labels at one step as:
% % \begin{equation}
% %     \tilde{f}(x^t)_{\tilde{y}^t} := \max_j \hat{f}(x^t)_{y^t_j},
% % \end{equation}
% Then we modify the heuristic notion of confidence for the entire sequence:
% \begin{equation}
%     \tilde{f}(\olsi{x})_{\tilde{y}} := \min_t \max_j \hat{f}(x^t)_{y^t_j}.
% \end{equation}
% This means for each time step $t$, we are using the highest softmax value among the true labels. We continue with the usual conformalization procedure and first define the calibration scores:
% \begin{equation}
%     \tilde{s}_i := 1-\tilde{f}(\olsi{x})_{\tilde{y}}, i=1,...,N.
% \end{equation}

% Again, define $\tilde{q}$ to be the $\frac{\lceil (n+1)(1-\alpha) \rceil}{n}$ empirical quantile of $\tilde{s}_1, ..., \tilde{s}_n$. For a new test sequence, define:
% \begin{equation}
%     \tilde{C}(\olsi{x}_\text{test}) := \{ \tilde{y} \ | \ \tilde{f}(\olsi{x}_\text{test})_{\tilde{y}} \geq 1-\tilde{q} \}.
% \end{equation}

% Note here $\tilde{C}(\olsi{x}_\text{test})$ is a bit different from $\olsi{C}(\olsi{x}_\text{test})$: they are both a set of prediction sequences, but for each prediction in the sequence, while $\olsi{C}(\olsi{x}_\text{test})$ contains a single one, now $\tilde{C}(\olsi{x}_\text{test})$ can contain multiple ones (\eg \{(\{a,b\},\{b,c\},\{a,c\}), (\{b\},\{b,c\},\{c\}), ...\} with $T=3$). In practice, we need something in the form of $\olsi{C}(\olsi{x}_\text{test})$ instead, since we do not have a principled way of outputting a prediction set from softmax values before calibration. 

% Suppose $\tilde{y}_\text{test} \in \tilde{C}(\olsi{x}_\text{test})$. By definition of $\tilde{C}(\olsi{x}_\text{test})$,
% \begin{align}
%     \tilde{f}(\olsi{x}_\text{test})_{\tilde{y}} &\geq 1-\tilde{q}, \\
%     \min_t \max_j \hat{f}(x^t)_{y^t_j} &\geq 1-\tilde{q}, \\
%     \max_j \hat{f}(x^t)_{y^t_j} &\geq 1-\tilde{q}, \forall t \\
% \end{align}

% Now define $\tilde{y}'_\text{test} := \{y \ | \ \underset{j}{\max} \ \hat{f}(x^t)_{y^t_j} \ \forall \tilde{y}^t \in \tilde{y}_\text{test} \}$, then:
% \begin{equation}
%     \forall{t} \ , \tilde{y}_\text{test} \in C^t(x^t_\text{test}).
% \end{equation}

% Conformal prediction then provides a bound on $\PP(\tilde{y} \notin \olsi{C}(\tilde{x}_\text{test}))$ when $\tilde{x}_\text{test}$ is drawn from the same distribution as the calibration sequences.

\subsection{Conditional coverage guarantee}

Calibrate once with a particular calibration dataset, and then the coverage guarantee holds over test samples with high probability; the original conformal prediction coverage is marginal, which means it holds over both sampling the calibration dataset and test samples.


==> old/sections/related.tex <==
\section{Related work}


==> old/sections/settings.tex <==
\section{Robot asking for help}

Types of guarantees

Prompt details, ...


==> sections/background.tex <==
\section{Background: Conformal Prediction}
\label{sec:background}

% Conformal Prediction (CP) is a distribution-free technique to make uncertainty set predictions for any black-box predictor. This method can be applied to any model that makes point predictions (or heuristic uncertainty set predictions), including regressors and classifiers. Intuitively, the CP algorithm involves evaluating the \textit{nonconformity score} as a measure of how good the model predictions are in comparison to the true label for an exchangeable dataset. The algorithm then provides a prediction set such that, for a \textit{new} prediction, this set holds with the desired probability level.

% Suppose we are given a model $\mathcal{R}$ and we obtain $n$ i.i.d. samples $(U_1, U_2, \dotsc U_n)$ of the nonconformity score such that if the disagreement between the model prediction and the true label increases, the nonconformity score increases. Using conformal prediction, we get the following bound on the next i.i.d. sample given the desired miscoverage level, $\alpha$,
% \begin{equation*}
%     \mathbb{P}(U_{n+1} \leq \hat{q}_{1-\alpha}) \geq 1-\alpha
% \end{equation*}
% where, we use the order statistics $U_{(1)}, U_{(2)}, \dotsc U_{(n)}$, to obtain the prediction set for the $(n+1)^{\text{th}}$ sample by computing the quantile,
% \begin{equation*}
%     \hat{q}_{1-\alpha} = \left\{ \begin{array}{ll}
%          U_{(\lceil(n+1)(1-\alpha)\rceil)}, \quad & \text{if} \lceil(n+1)(1-\alpha)\rceil \leq n \\
%          \infty, & \text{otherwise}
%     \end{array}\right.
% \end{equation*}

% This is a relatively straightforward framework to obtain prediction sets. We don't make any assumptions on the underlying distribution of the samples nor do we need to assume that the samples are i.i.d. (we do so above for simplicity, in fact exchangeability of the calibration and training dataset is enough).  The design problem is how we set up the nonconformity score $U$. Let's look at regression and classification examples (we assume for simplicity of presentation that the input is one-dimensional):
% \begin{itemize}
    % \item \textbf{Regression: }Suppose we have input/output pairs $(X_1, Y_1), (X_2, Y_2), \dotsc, (X_n, Y_n) \in \mathbb{R}\times \mathbb{R}$. The regression module, $\mathcal{R}$, makes predictions $f:\mathbb{R}\rightarrow\mathbb{R}$. The nonconformity score is defined as the difference between the true realization $Y$ and the point prediction $f(X)$. Hence, $U_i = \lVert f(X_i) - Y_i\rVert$.
%     \item \textbf{Classification: }Suppose we have input and output class pairs $(X_1, Y_1), (X_2, Y_2), \dotsc, (X_n, Y_n) \in \mathbb{R}\times\{1, 2, \dotsc K\}$, where the output label $Y$ is represented using the index set. The classification module, $\mathcal{R}$, makes predictions of the likelihood of each class $f:\mathbb{R}\rightarrow[0,1]^K$ such that $f(X_i)_{Y_i}$ is the predicted likelihood of the true class $Y_i$ of the input $X_i$. Hence, we can define the nonconformity score as $U_i = 1 - f(X_i)_{Y_i}$.
% \end{itemize}


% ----

% \begin{itemize}
%     \item Brief overview of conformal prediction: set-based predictors, calibration procedure, marginal coverage, conditional coverage.
%     \item Highlight: no assumptions on distribution, works with black-box predictor (with uncalibrated confidence), provides guarantees.
% \end{itemize}

==> sections/implementation.tex <==
\section{Implementation Details}
\label{sec:implementation}

\begin{itemize}
    \item All the other stuff we didn't describe (e.g., perception pipeline, low-level policy implementation, etc.).
    \item \allen{general setup for prompting}
    % \item \allen{human help: clarification and providing answers.}
\end{itemize}

==> sections/token-prediction.tex <==
\section{Assessing LLM Confidence through Multiple Choice Question Answering}
\label{sec:mcqa}

\allen{Andy: It seems the savetrees package makes the $\hat{f}$ notation look off. Do you know an easy way to fix it?}

In order to assess how uncertain the LLM is about different possible actions to take given the context, we need to first define (1) the space $\mathcal{Y}$ of possible plans that the LLM predicts, and (2) the model's ``confidence'' $\hat{f}(x)_y$ in each prediction $y \in \mathcal{Y}$ given the context $x$. In this work, we propose formulating LLM planning as Multiple Choice Question Answering (MCQA) to design $\mathcal{Y}$ and evaluate $\hat{f}(x)_y$. This will allow us to achieve uncertainty alignment using conformal prediction in~\cref{sec:approach}. Planning as MCQA involves two steps (\cref{fig:mcqa-cp}): %, and helps achieve uncertainty alignment using conformal prediction in Sec.~\ref{sec:approach}.
% One straightforward way is to use the space of all possible sequences of tokens for (1), and the probability associated with them for (2): (auto-regressive) LLM models the probability of a sentence output $W=\{w_0, w_1, ..., w_m\}, w \in \mathcal{W}$,
% % , a sequence of individual tokens, 
% as $p(W) = \prod_{j=0}^m p(w_j|w_{<j})$, where $w_{<j}$ denotes all tokens before $j$th one including the context. 
% There are two main challenges though. First, the set of possible outputs is exponentially large, $O(|\mathcal{W}|^m)$ ---
% % , where $\mathcal{W}$ is the set of possible tokens. 
% % Outputs such as ``put the yellow block on the blue block`` and ``place the yellow cube on top of the blue block``, are semantically equivalent but possibly assigned with non-trivially different probabilities given the same context \citep{}. 
% % Also 
% it is infeasible to acquire the probabilities of all possible outputs. Second, it is known \citep{} that 
% % the product of conditional probability 
% $p(W)$ or the similar perplexity metric \citep{} assigns lower confidence to longer $W$. For example, it may bias against the action ``grab a bottle of fresh orange juice from the fridge'' than ``grab a sandwich from the fridge'' even when the human asks for something to drink. In Sec.~\ref{?} we show in experiments that the perplexity metric leads to worse uncertainty calibration.


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/mcqa-cp.pdf}
    \caption{\knowno formulates LLM planning as Multiple Choice Question Answering (MCQA) by first prompting LLM to generate plausible options and then asking it to predict the correct one. Using the next-token likelihoods collected with a calibration dataset, conformal prediction provides the quantile value $\hat{q}$ that determines the options included in the prediction set in a test scenario.
    % \allen{I made a draft. }
    }
    \label{fig:mcqa-cp}
    \vspace{-10pt}
\end{figure}

% To better quantify the uncertainty of the LLM-based planner over possible actions, 
% In this work, we propose formulating LLM planning as Multiple Choice Question Answering (MCQA) to better design $\mathcal{Y}$ and $\hat{f}(x)_y$. It involves two steps (Fig.~\ref{fig:mcqa}):
\begin{enumerate}[leftmargin=*]
    \item Multiple-choice generation: given the context $x^t$, the LLM is prompted to generate a diverse set of candidate plans
    % For example, LLM generates four options
    labeled with `$A$', `$B$', `$C$', `$D$'\footnote{In Appendix \ref{?} we detail the post-processing of the LLM output to extract the four options.}, and an additional possible plan, `$E) \ \text{an option not listed here}$', which is appended post-hoc. These options are added to the current context $x^t$ to form the augmented context $\tilde{x}^t$.
    % Such sentence generation eliminates the bias against longer sentence.
    \item Next-token prediction: the same LLM is asked to choose among the options. Thus the LLM's confidence in each option is modeled as the conditional probability of the LLM predicting the corresponding label, i.e., $\hat{f}(\tilde{x}^t)_y = p(y|\tilde{x}^t), \ y \in \{\textrm`A\textrm', \textrm`B\textrm', \textrm`C\textrm', \textrm`D\textrm', \textrm`E\textrm'\}$.
    % We obtain the probability of the LLM outputting each token of $\{\textrm`A\textrm', \textrm`B\textrm', \textrm`C\textrm', \textrm`D\textrm', \textrm`E\textrm'\}$, e.g., $p_A= p(\textrm`A\textrm'|x^t)$. 
    % They act as the LLM's confidence in each generated option. 
    % It is known that LLM can generate well-calibrated (less biased) probabilities in next-token prediction \citep{}.
\end{enumerate}

Effectively, we augment the original input with the multiple choices generated based on it, resulting in the prediction space $\mathcal{Y} = \{\textrm`A\textrm', \textrm`B\textrm', \textrm`C\textrm', \textrm`D\textrm', \textrm`E\textrm'\}$\footnote{We differentiate the prediction space $\mathcal{Y}$ from the per-token output space $\mathcal{W}$. While the LLM can output any token from $\mathcal{W}$, we are only concerned with the probabilities of LLM predicting $y \in \mathcal{Y}$.}. % The correct plan for the context is converted to the true label in $\mathcal{Y}$ if the plan matches any of the generated options; if not, the true label is `E'.
% We use the next-token probability as the model confidence, $p_y = \hat{f}_y, y \in \mathcal{Y}$.
Such a design affords three benefits.
% \vspace{-5pt}
% \begin{itemize}[leftmargin=*]
%     \item 
    % If instead we consider LLM predictions on sentence level, then $\mathcal{Y}$ can 
    % contain semantically equivalent phrases,
    % We want to avoid the LLM predicting semantically equivalent phrases
    % such as ``open the top drawer and put the sponge in it'' and ``put the sponge in the top drawer by first opening it'' since they can be assigned with non-trivially different probabilities given the same context \cite{} and thus introducing bias. We find that multiple-choice generation by prompting can effectively generate a set of plans that are semantically different.
    First, through multiple-choice generation, we eliminate choices that the LLM deems improbable. By initially prompting the LLM to generate its own options, we avoid the need to assess the probability of each potential plan, including those that are highly unlikely given a particular context.
    % Multiple-choice generation eliminates options that the LLM considers as low probability options. By prompting the LLM to generate options on its own first, we do not need to evaluate the probability of every possible plan given a context.
    % with few-shot prompting leads to diverse set of candidate actions that are structured and semantically different.
    % they can be assigned with non-trivially different probabilities given the same context.
    % By prompting the LLM to generate diverse and semantically different plans, 
    % The original prediction space of the LLM is unconstrained and exponentially large, $O(|\mathcal{W}|^m)$, where $\mathcal{W}$ is the set of possible tokens and $m$ is the maximum token length. It would be infeasible to acquire $f(x)_y$ for every possibly $y$.
    Second, LLMs are often better at \emph{evaluating} options as compared to generating them; MCQA allows us to utilize this ability in order to rank generated options (for use by conformal prediction).  
    Third, it is known that LLMs tend to assign lower probabilities to longer outputs. Next-token prediction eliminates this bias due to varying lengths \citep{murray2018correcting}.
    % the probability $p(W)$ or the similar perplexity metric \citep{} assigns lower confidence to longer $W$.
    In~\cref{subsec:saycan} we show in experiments that 
    % the perplexity metric
    using sentence-level probabilities leads to worse uncertainty calibration.
% \end{itemize}

% \sumeet{There is some fuzziness here in the distinction between LLM uncertainty and task success. By always choosing option `E', and triggering human help, one can achieve a 100$\%$ success rate. It may be worthwhile to add a comment/remark here about the fact that `E' is necessary to include to ensure that there is always a `correct' option, as far as CP is concerned. One can then differentiate the results conditional on whether or not `E' \emph{was} the correct option for a given list of LLM generated plans. This allows the separation of two issues: (i) whether the LLM generated correct plans within options `A' - `D', and (ii) the uncertainty associated with multiple correct plans. If plans `A' - `D' are all wrong, then it may be ``certain" about its mistake, and ask for help via `E', albeit, and importantly, a different mode of asking for help. This would not be measurable nor controllable via CP.}

% By adding the additional option `an option not listed here', we ensure that the true label is always present among the options.

% Effectively we reduce the problem of ranking possible solutions to next-token prediction to obtain unbiased probabilities, and then putting the model in "verify" (i.e. critic) mode to capture uncertainty.

% \allen{there are some details about how to better generate multiple choices through one-shot prompting that might worth talking about here}

% Difficult to apply CP on sentence-level output - event class is exponentially large. Decide to use multiple choice question answering + next-token prediction.

% Conformal prediction assumes that the LLM planner returns meaningful uncalibrated scores for each step of the plan.
% For image classification, this is as simple as the class category softmax scores, but for LLMs this is a bit more tricky. LLM planners are usually autoregressive models, which means they predict each step token by token. We can get softmax scores for each token. But to get a single score for a sequence of tokens, we need perplexity. However, perplexity is a poor scoring function because it biases against longer steps with lower values.

% \paragraph{Label.} For each step, there is at least one true action. To always cover the true action with the multiple choices at each step, we will consider four options generated with the template or by prompting, plus a fifth option ``none of the other options''. By assigning higher biases to tokens of $[a, b, c, d ,e]$ (with \verb|logit_bias| argument in \verb|openai.Completion.create()| function for GPT-3) and setting the maximum length to be 1, we can constrain the LLM to always output one of the five letters. We define the label of each prediction as the true option among the five, denoted $y$. We will extend to multi-label setting later.
